Tensors, !-graphs, and non-commutative quantum structures (extended version)

!-graphs provide a means of reasoning about infinite families of string diagrams and have proven useful in manipulation of (co)algebraic structures like Hopf algebras, Frobenius algebras, and compositions thereof. However, they have previously been limited by an inability to express families of diagrams involving non-commutative structures which play a central role in algebraic quantum information and the theory of quantum groups. In this paper, we fix this shortcoming by offering a new semantics for non-commutative !-graphs using an enriched version of Penrose's abstract tensor notation.

==> oldproofs.tex <==
  % \begin{proof} (Sketch)
  %   Again we need only check the conditions F1-2, C1-3:
  %   \begin{itemize}
  %     \item[F1-2:]  Trivial since any new edges/boxes are fresh ones which can only have come from the distinct edges/boxes in $G$.
  %     \item[C1:] Edges in $\Exp_A(G)$ are either edges from $G$ or fresh names for edges in $G$. For the former $\ectx, \nctx$ have not been changed so the condition holds. For the later we know from Lemma~\ref{lem:contexts} that boxes in $\ectx, \nctx$ have only been removed or replaced by fresh versions of themselves hence still distinct.
  %     \item[C2:] For $a\in\Edges(G)$ (writing $B'$ for $\fr(B)$):
  %       \begin{itemize}
  %         \item[$\bullet$] $\ectx_{\Exp_A(G)}(a) = [E_1,\ldots,E_n]=\ectx_G(a)$ and $E_i\prec_G E_{i+1} \implies E_i\prec_{\Exp_A(G)} E_{i+1}$ so the condition holds.
  %         \item[$\bullet$] $\ectx_{\Exp_A(G)}(\fr(a)) = [E_1',\ldots,E_i',E_{i+1},\ldots,E_n]$ for some $E_i$. \\
  %         $E_i'$ must have been created inside $E_{i+1}$ in $\Exp_A(G)$. \\
  %         For others it is clear that $j<i \implies E_j'\prec_{\Exp_A(G)} E_{j+1}'$, \\
  %         $j>i \implies E_j\prec_{\Exp_A(G)} E_{j+1}$.
  %       \end{itemize}
  %     \item[C3:] For $\eout{a},\ein{a}\in\Edges(\Exp_A(G))$ s.t $\eout{a},\ein{a}\in\Edges(G)$ then $\ectx, \nctx$ were not affected by $\Exp_A$ so the condition still holds. \\
  %     For $\eout{\fr(a)},\ein{\fr(a)}\in\Edges(\Exp_A(G))$ s.t $\eout{a},\ein{a}\in\Edges(G)$ \\
  %     then $\exists E_i,N_i \in \boxnames$ s.t \\
  %     $[E_1,\ldots,E_n].\nctx_G(\ein{a})=\ectx_G(\eout{a}).[N_1,\ldots,N_m]$\\
  %     $[E_1,\ldots,E_n].\nctx_G(\eout{a})=\ectx_G(\ein{a}).[N_1,\ldots,N_m]$\\
  %     We have four cases to check for how $\ectx,\nctx$ are affected by $\Exp_A$:
  %     \begin{itemize}
  %       \item[$\bullet$] $A\in \ectx_G(\ein{a})\cap \ectx_G(\eout{a})$ then $A=E_i$ for some $i$ and letting $es:=[E_1',\ldots,E_{i-1}',E_{i+1},\ldots,E_n]$ and $bs:=[N_1,\ldots,N_m]$ we have the condition holds.
  %       \item[$\bullet$] $A\in \nctx_G(\ein{a})\cap \nctx_G(\eout{a})$ then $A=N_i$ for some $i$ and letting $es:=[E_1',\ldots,E_m']$ and $bs:=[N_1',\ldots,N_{i-1}',N_{i+1},\ldots,N_n]$ we have the condition holds.
  %       \item[$\bullet$] $A\in \ectx_G(\ein{a})\cap \nctx_G(\eout{a})$ then letting $es:=[E_1',\ldots,E_m']$ and $bs:=[N_1,\ldots,N_m]$ we have the condition holds.
  %       \item[$\bullet$] $A\in \nctx_G(\ein{a})\cap \ectx_G(\eout{a})$ similar to previous case.
  %     \end{itemize}
  %   \end{itemize}
  % \end{proof}

  % \begin{theorem}
  %   If in graph $G$, box $B$ is nested inside box $A$ ($B\prec_G\ldots\prec_G A$) then we can find a freshness function $\fr'$ s.t. the following equations hold on $G$:
  %   \begin{align*}
  %     \Kill_{A} \circ \Op_{B,\fr_B} &= \Kill_{A} \\
  %     \Drop_{A} \circ \Op_{B,\fr_B} &= \Op_{B,\fr_B} \circ \Drop_{A} \\
  %     \Exp_{A,\fr_A} \circ \Op_{B,\fr_B} &= \Op_{B',\fr'} \circ \Op_{B,\fr_B} \circ \Exp_{A,\fr_A} \\
  %     \Copy_{A,\fr_A} \circ \Op_{B,\fr_B} &= \Op_{B',\fr'} \circ \Op_{B,\fr_B} \circ \Copy_{A,\fr_A}
  %   \end{align*}
  % \end{theorem}
  % \begin{proof} %Sketch
  %   (Sketch) Induction on $\edgeterms$ and $\graphterms$. The interesting cases are $\term{[e>C}$, $\term{<e]C}$ and $\term{[G]C}$ where $C=A,B$. These can be checked explicitly. The freshness function $\fr'$ only requires that $\fr_A(x)\mapsto\fr_A(\fr_B(x))$.
  % \end{proof}

  % \begin{proof}
  %   Proofs are done inductively on edgeterms and graphterms and so the only interesting cases are $\term{[e>C}$, $\term{<e]C}$ and $\term{[G]C}$ where $C$ is either $A$ or $B$. \\
  %   $\Kill_A \circ \Op_B = \Kill_A$:
  %   \begin{itemize}
  %     \item $\Kill_A \circ \Op_B \term{[e>A} = \Kill_A \term{[\Op_B(e)>A} = \epsilon$ \\
  %       $\Op_B \circ \Kill_A \term{[e>A} = \Op_B(\epsilon) = \epsilon$
  %     \item $\term{<e]C}$ case is similar to previous case.
  %     \item $\Kill_A \circ \Op_B \term{[G]A} = \Kill_A \term{[\Op_B(G)]A} = 1$ \\
  %       $\Op_B \circ \Kill_A \term{[G]A} = \Op_B (1) = 1$
  %   \end{itemize}
  %   $\Drop_A \circ \Op_B = \Op_B \circ \Drop_A$:
  %   \begin{itemize}
  %     \item $\Drop_A \circ \Op_B \term{[e>A} = \Drop_A \term{[\Op_B(e)>A} = \Op_B(e)$ \\
  %       $\Op_B \circ \Drop_A \term{[e>A} = \Op_B(e)$
  %     \item $\term{<e]C}$ case is similar to previous case.
  %     \item $\Drop_A \circ \Op_B \term{[G]A} = \Drop_A \term{[\Op_B(G)]A} = \Op_B(G)$ \\
  %       $\Op_B \circ \Drop_A \term{[G]A} = \Op_B (G)$
  %   \end{itemize}
  %   $\Exp_A \circ \Op_B = \Op_{B'} \circ \Op_B \circ \Exp_A$:
  %   \begin{itemize}
  %     \item \begin{align*}
  %         \Exp_A \circ \Op_B \term{[e>A} &= \Exp_A \term{[\Op_B(e)>A} \\
  %         &= \term{[\Op_B(e)>A}\fr_A(\Op_B(e))
  %       \end{align*}
  %       \begin{align*}
  %         \Op_{B'} \circ \Op_B \circ \Exp_A \term{[e>A} &= \Op_{B'} \circ \Op_B (\term{[e>A}\fr_A(e)) \\
  %         &= \term{[\Op_B(e)>A}\Op_{B'}(\fr_A(e))
  %       \end{align*}
  %       Any freshness function s.t $\fr_A(x)\mapsto\fr_A(\fr_B(x))$ works for $\Op_{B'}$.
  %     \item $\term{<e]C}$ case is similar to previous case.
  %     \item \begin{align*}
  %         \Exp_A \circ \Op_B \term{[G]A} &= \Exp_A \term{[\Op_B(G)]A} \\
  %         &= \term{[\Op_B(G)]A}\fr_A(\Op_B(G))
  %       \end{align*}
  %       \begin{align*}
  %         \Op_{B'} \circ \Op_B \circ \Exp_A \term{[G]A} &= \Op_{B'} \circ \Op_B (\term{[G]A}\fr_A(G)) \\
  %         &= \term{[\Op_B(G)]A}\Op_{B'}(\fr_A(G))
  %       \end{align*}
  %       Any freshness function s.t $\fr_A(x)\mapsto\fr_A(\fr_B(x))$ works for $\Op_{B'}$.
  %   \end{itemize}
  %   $\Copy_A \circ \Op_B = \Op_{B'} \circ \Op_B \circ \Copy_A$:
  %   \begin{itemize}
  %     \item \begin{align*}
  %         \Copy_A \circ \Op_B \term{[e>A} &= \Copy_A \term{[\Op_B(e)>A}\\
  %         &= \term{[\Op_B(e)>A[\fr_A(\Op_B(e))>{\fr_A(A)}}
  %       \end{align*}
  %       \begin{align*}
  %         \Op_{B'} \circ \Op_B \circ \Copy_A \term{[e>A} &= \Op_{B'} \circ \Op_B (\term{[e>A[\fr_A(e)>{\fr_A(A)}})\\
  %         &= \term{[\Op_B(e)>A[\Op_{B'}(\fr_A(e))>{\fr_A(A)}}
  %       \end{align*}
  %       Any freshness function s.t $\fr_A(x)\mapsto\fr_A(\fr_B(x))$ works for $\Op_{B'}$.
  %     \item $\term{<e]C}$ case is similar to previous case.
  %     \item \begin{align*}
  %         \Copy_A \circ \Op_B \term{[G]A} &= \Copy_A \term{[\Op_B(G)]A}\\
  %         &= \term{[\Op_B(G)]A[\fr(\Op_B(G))]{\fr(A)}}
  %       \end{align*}
  %       \begin{align*}
  %         \Op_{B'} \circ \Op_B \circ \Copy_A \term{[G]A} &= \Op_{B'} \circ \Op_B (\term{[G]A[\fr_A(G)]{\fr_A(A)}})\\
  %         &= \term{[\Op_B(G)]A[\Op_{B'}(\fr_A(G))]{\fr_A(A)}}
  %       \end{align*}
  %       Any freshness function s.t $\fr_A(x)\mapsto\fr_A(\fr_B(x))$ works for $\Op_{B'}$.
  %   \end{itemize}
  %   There is one problem with finding $\fr'$. This is in the case where $\Op_B$ deleted a free variable and then $\Exp_A$ or $\Copy_A$ brought it back. In that case $\fr'$ is not a valid freshness function.
  % \end{proof}


  % We also expect that any of our defined !-box operations preserves equality. So we get a rule for each $\Op\in\{\Kill,\Drop,\Exp,\Copy\}$:

 %  \begin{prooftree}
 %    \AxiomC{$G=H$}
 %    \RightLabel{\scriptsize($\Op_A$)}
 %    \UnaryInfC{$\Op_A(G=H)$}
 %  \end{prooftree}

 %  We can use these rules to produce more rules such as a second product rule:
 %  \begin{theorem}\qquad
 %    \begin{prooftree}
 %      \AxiomC{$G=G'$}
 %      \RightLabel{\scriptsize(Prod2)}
 %      \UnaryInfC{$HG=HG'$}
 %    \end{prooftree}
 %  \end{theorem}
 %  \begin{proof}
 %    \begin{prooftree}
 %      \AxiomC{$G=G'$}
 %      \RightLabel{\scriptsize(Prod)}
 %      \UnaryInfC{$GH=G'H$}
 %      \RightLabel{\scriptsize($\equiv$)}
 %      \UnaryInfC{$HG=HG'$}
 %    \end{prooftree}
 %  \end{proof}

 %  We can also derive a stronger weakening rule:
 %  \begin{theorem}\qquad
 %    \begin{prooftree}
 %      \AxiomC{$G=G'$}
 %      \AxiomC{$K=K'$}
 %      \RightLabel{\scriptsize(Weak')}
 %      \BinaryInfC{$\Weak_{A\to K}(G)=\Weak_{A\to K'}(G')$}
 %    \end{prooftree}
 %  \end{theorem}
 %  \begin{proof}
 %    Proof by induction on the complexity of $G'$ that
 %    \begin{prooftree}
 %      \AxiomC{$K=K'$}
 %      \RightLabel{\scriptsize}
 %      \UnaryInfC{$\Weak_{A\to K}(G')=\Weak_{A\to K'}(G')$}
 %    \end{prooftree} then transitivity gives the desired result.
 %    \begin{itemize}
 %      \item $G'=\phi_e,1$ trivial
 %      \item $G'=\gbox{H}{B}$ with $B\not=A$
 %      \begin{prooftree}
 %        \AxiomC{$K=K'$}
 %        \RightLabel{\scriptsize(IH)}
 %        \UnaryInfC{$\Weak_{A\to K}(H)=\Weak_{A\to K'}(H)$}
 %        \RightLabel{\scriptsize(Box)}
 %        \UnaryInfC{$\gbox{\Weak_{A\to K}(H)}{B}=\gbox{\Weak_{A\to K'}(H)}{B}$}
 %        \RightLabel{\scriptsize($\equiv$)}
 %        \UnaryInfC{$\Weak_{A\to K}(\gbox{H}{B})=\Weak_{A\to K'}(\gbox{H}{B})$}
 %      \end{prooftree}
 %      \item $G'=\term{[H]A}$
 %      \begin{prooftree}
 %        \AxiomC{$K=K'$}
 %        \RightLabel{\scriptsize(Prod)}
 %        \UnaryInfC{$HK=HK'$}
 %        \RightLabel{\scriptsize(Box)}
 %        \UnaryInfC{$\gbox{HK}{A}=\gbox{HK'}{A}$}
 %        \RightLabel{\scriptsize($\equiv$)}
 %        \UnaryInfC{$\Weak_{A\to K}(\term{[H]A})=\Weak_{A\to K'}(\term{[H]A})$}
 %      \end{prooftree}
 %      \item $G'=H_1H_2$ \\
 %      Writing $W_K$ for $\Weak_{A\to K}$:
 %      \begin{prooftree}
 %        \AxiomC{$K=K'$}
 %        \RightLabel{\scriptsize(IH)}
 %        \UnaryInfC{$W_K(H_1)=W_{K'}(H_1)$}
 %        \AxiomC{$K=K'$}
 %        \RightLabel{\scriptsize(IH)}
 %        \UnaryInfC{$W_K(H_2)=W_{K'}(H_2)$}
 %        \RightLabel{\scriptsize(Prod)}
 %        \BinaryInfC{$W_K(H_1H_2)=W_{K'}(H_1H_2)$}
 %      \end{prooftree}
 %    \end{itemize}
 %  \end{proof}

  % \begin{theorem}
  %   Let $\fr$ be a freshness function for two !-tensor expressions $G, H$. Then $G\equiv H$ implies $\Op_{B,\fr}(G) \equiv \Op_{B,\fr}(H)$.
  % \end{theorem}
 %  \begin{proof}
 %    We need to check our enforced equivalences still hold after $\Op_B$:
 %    \begin{itemize}
 %      \item $\Op_B(1G)\equiv\Op_B(1)\Op_B(G)\equiv1\Op_B(G)\equiv\Op_B(G)\equiv\ldots\equiv\Op_B(G1)$
 %      \item $\Op_B(\epsilon e)\equiv\Op_B(\epsilon)\Op_B(e)\equiv\epsilon\Op_B(e)\equiv\Op_B(e)\equiv\ldots\equiv\Op_B(e\epsilon)$
 %      \item $\term{\Op_B([\epsilon>A)}\equiv\term{[\Op_B(\epsilon)>A}\equiv\term{[\epsilon>A}\equiv\ldots\equiv\term{\Op_B(<\epsilon]A)}$ \quad if $A\not\equiv B$ \\
 %      When $A\equiv B$ we need to check each operation individually but they are all easy to show
 %      \item For products:
 %        \begin{align*}
 %          \Op_A(G H) &\equiv \Op_A(G)\Op_A(H) \\
 %          &\equiv \Op_A(H)\Op_A(G) \\
 %          &\equiv \Op_A(H G)
 %        \end{align*}
 %      \item Given $a\in\Bound(G)$ and $b\notin\Edges(G)$
 %        %Todo
 %        % \begin{align*}
 %        %   \Op(G[a\mapsto b]) &\equiv \Op(G)[a\mapsto b,\fr(a)\mapsto \fr(b)] \\
 %        %   &\equiv \Op(G) \\
 %        %   &\equiv \Op(G)
 %        % \end{align*}
 %    \end{itemize}
 %  \end{proof}

 %  \begin{theorem}
 %    If $A\not=B$ are not nested inside each other then any !-box operations $\Op_A, \Op'_B$ commute.
 %  \end{theorem}
 %  \begin{proof}
 %    (Sketch) Each operation only affects a graph locally at their respective boxes which has no effect on the other box.
 %  \end{proof}

 %  \begin{corollary}
 %    Any string of operations on a graph $G$ can be written in a normal form where all top level box operations (ordered by !-box name) are applied first then all operations on first level children (ordered by !-box name) and so on.
 %  \end{corollary}

 %  \begin{proof}
 %    (Sketch) Take the first top level box, $A$ in $G$ then use the previous theorems to move operations on $A$ to be first. This only creates finitely many extra operations on boxes nested in $A$. Applying the same to the rest of the top level boxes we get them all first and in order so we can ignore them and recursively normalise the order on what is left.
 %  \end{proof}
